An Iterative Mechanism for Coupling Electricity Markets

The coordinated operation of interconnected but locally controlled electricity markets is generally referred to as a "coupling". In this paper we propose a new mechanism design for efficient coupling of independent electricity markets. The mechanism operates after each individual market has settled (e.g. hour-ahead) and based upon the reported supply and demand functions for internal market optimization (clearing), each market operator is asked to iteratively quote the terms of energy trade (on behalf of the agents participating in its market) across the transmission lines connecting to other markets. The mechanism is scalable as the informational demands placed on each market operator at each iteration are limited. We show that the mechanism's outcome converges to the optimal flows between markets given the reported supply and demand functions from each individual market clearing. We show the proposed market coupling design does not alter the structure of incentives in each internal market, i.e., any internal market equilibrium will remain so (approximately) after coupling is implemented. This is achieved via incentive transfers (updated at each iteration) that remunerate each market with its marginal contribution (i.e. cost savings) to all other participating markets. We identify a sufficient condition on a uniform participation fee for each market operator ensuring the mechanism incurs no deficit. The proposed decentralized mechanism is implemented on the three-area IEEE Reliability Test System where the simulation results showcase the efficiency of proposed model.

==> macro.tex <==
\usepackage{amsmath}
\usepackage{mathrsfs}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{graphicx}
\usepackage{enumitem}
%\usepackage{epstopdf}
\usepackage{subfigure}
\usepackage{color}
\usepackage{multirow}
\usepackage{verbatim}
%\usepackage{galois}
\usepackage{algorithm,algorithmicx,algpseudocode}
\usepackage{cite}
\usepackage{bbm}
\usepackage{bigstrut}
\usepackage[left=1in,top=1in,right=1in,bottom=1in,letterpaper]{geometry}
\usepackage[linktocpage,colorlinks,linkcolor=blue,anchorcolor=blue,citecolor=blue,urlcolor=blue]{hyperref}
\usepackage{cleveref}

\providecommand{\keywords}[1]
{\small	
  \textbf{\textit{Keywords---}} #1
}

%\makesavenoteenv{tabular}
%\makesavenoteenv{table}
\numberwithin{equation}{section}

\newtheorem{theorem}{Theorem}[section]
\crefname{theorem}{Theorem}{Theorems}

\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\crefname{lemma}{Lemma}{Lemmas}

\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
\crefname{definition}{Definition}{Definitions}

\newtheorem{fact}[theorem]{Fact}
\newtheorem{example}{Example}[section]
\newtheorem{assumption}{Assumption}
\crefname{assumption}{Assumption}{Assumptions}

\newtheorem{remark}[theorem]{Remark}
\newtheorem{question}{Question}[section]
%\linespread{1.6}

\newcommand{\A}{\mathcal{A}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\G}{\mathcal{G}}
\newcommand{\J}{\mathcal{J}}

\newcommand{\calL}{\mathcal{L}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\N}{\mathcal{N}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cL}{\mathcal{L}}

\newcommand{\U}{\mathcal{U}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\W}{\mathcal{W}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cX}{\mathcal{X}}

\newcommand{\bD}{\mathbf{D}}
%\newcommand{\ba}{\mathbf{a}}


\newcommand{\R}{\mathbb{R}}
%\newcommand{\E}{\mathbb{E}}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\newcommand{\etal}{ et al. }
\newcommand{\br}{\mathbb{R}}
\newcommand{\RR}{\mathbb{R}}
%\newcommand{\Proj}{{\rm Proj}}
\newcommand{\half}{\frac{1}{2}}

\newcommand{\X}{\mathbf{X}}
\newcommand{\bx}{\mathbf{x}}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\bad}{\begin{aligned}}
\newcommand{\ead}{\end{aligned}}
%\renewcommand{\arraystretch}{0.8}%
\newcommand{\normone}[1]{\| #1 \|_1}
\newcommand{\normtwo}[1]{\| #1 \|}
\newcommand{\abs}[1]{| #1 |}
\newcommand{\norminf}[1]{\| #1 \|_{\infty}}
\newcommand{\normfro}[1]{\| #1 \|_{\text{F}}}
\newcommand{\inp}[2]{\left\langle #1, #2 \right\rangle}
%\newcommand{\setword}[2]{\phantomsection #1\def\@currentlabel{\unexpanded{#1}}\label{#2}}
\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand{\lineSearch}{\mathop{\rm line\_search}}
\newcommand{\Line}{\mathop{\rm Line}}

\newcommand{\p}{\mathcal{P}}
\newcommand{\ps}{\mathcal{P_{\St}}}
\newcommand{\pt}{\mathcal{P_{\T}}}

\newcommand{\psm}{\mathbf{Proj_{\St}}}
\newcommand{\dist}{\mathrm{dist}}


\newcommand{\heta}{\hat{\eta}}
\newcommand{\hzeta}{\hat{\zeta}}
\newcommand{\htau}{\hat{\tau}}
